Towards Understanding Neural Collapse: The Effects of Batch Normalization and Weight Decay

Neural Collapse (NC) is a geometric structure recently observed at the terminal phase of training deep neural networks, which states that last-layer feature vectors for the same class would "collapse" to a single point, while features of different classes become equally separated. We demonstrate that batch normalization (BN) and weight decay (WD) critically influence the emergence of NC. In the near-optimal loss regime, we establish an asymptotic lower bound on the emergence of NC that depends only on the WD value, training loss, and the presence of last-layer BN. Our experiments substantiate theoretical insights by showing that models demonstrate a stronger presence of NC with BN, appropriate WD values, lower loss, and lower last-layer feature norm. Our findings offer a novel perspective in studying the role of BN and WD in shaping neural network features.

==> custom_defs.tex <==
\usepackage{mdframed}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{amsthm}


\newif\ifdoublecol

\newtheorem{theorem}{Theorem}% [section]
\newtheorem{proposition}{Proposition}% [section]
\newtheorem{corollary}{Corollary}% [section]
\newtheorem{lemma}{Lemma}% [section]
\newtheorem{definition}{Definition}% [section]
\newtheorem{conjecture}{Conjecture}% [section]
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\propositionautorefname}{Proposition}
\newcommand{\definitionautorefname}{Definition}
\newcommand{\bg}{\boldsymbol{\gamma}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\V}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\NC}{\ensuremath{\mathcal{NC}}\xspace}
